Mixed-integer linear representability, disjunctions, and Chvatal functions --- modeling implications

Jeroslow and Lowe gave an exact geometric characterization of subsets of $\mathbb{R}^n$ that are projections of mixed-integer linear sets, also known as MILP-representable or MILP-R sets. We give an alternate algebraic characterization by showing that a set is MILP-R {\em if and only if} the set can be described as the intersection of finitely many {\em affine Chvatal inequalities} in continuous variables (termed AC sets). These inequalities are a modification of a concept introduced by Blair and Jeroslow. Unlike the case for linear inequalities, allowing for integer variables in Chvatal inequalities and projection does not enhance modeling power. We show that the MILP-R sets are still precisely those sets that are modeled as affine Chvatal inequalites with integer variables. Furthermore, the projection of a set defined by affine Chvatal inequalites with integer variables is still an MILP-R set. We give a sequential variable elimination scheme that, when applied to a MILP-R set yields the AC set characterization. This is related to the elimination scheme of Williams and Williams-Hooker, who describe projections of integer sets using \emph{disjunctions} of affine Chvatal systems. We show that disjunctions are unnecessary by showing how to find the affine Chvatal inequalities that cannot be discovered by the Williams-Hooker scheme. This allows us to answer a long-standing open question due to Ryan (1991) on designing an elimination scheme to represent finitely-generated integral monoids as a system of Chvatal inequalities \emph{without} disjunctions. Finally, our work can be seen as a generalization of the approach of Blair and Jeroslow, and Schrijver for constructing consistency testers for integer programs to general AC sets.

==> guanyi-result.tex <==
% !TEX root = ../journal-submission.tex

Still by Theorems~\ref{theorem:jeroslow-lowe}~and~\ref{theorem:mic-is-milp}, for MIC sets $S$ and $T$, there exist two sets of vectors $r(S) := \{r^S_1, \ldots, r^S_{t^S} \} \subseteq \mathbb{Z}^n, r(T) := \{r^T_1, \ldots, r^T_{t^T} \} \subseteq \mathbb{Z}^n$ that give a characterization of $S$ and $T$ according to \eqref{eq:jeroslow-lowe-chraracterization}; that is,
\begin{align*}
S & = \bigcup_{i=1}^{k^S} P^S_i + \intcone \left\{r^S_1, \ldots, r^S_{t^S} \right\}. \\
T & = \bigcup_{i=1}^{k^T} P^T_i + \intcone \left\{r^T_1, \ldots, r^T_{t^T} \right\}.
\end{align*}
Since $S$ and $T$ satisfy $\rec S = \rec T$, then $\cone \left\{ r^S_1, \ldots, r^S_{t^S} \right\} = \cone \left\{ r^T_1, \ldots, r^T_{t^T} \right\}$. Thus $\cone \{r(T)\}$ and $\cone \{r(S)\}$ have the same set of extreme rays. Let $e$ be an extreme ray of $\cone \{r(T)\}$ and $\cone \{r(S)\}$. For $r(S)$ and $r(T)$, there exist two sets of vectors $R^S_e = \{r^S_{i_1}, \ldots, r^S_{i_s}\} \subseteq r(S)$ and $R^T_e = \{r^T_{j_1}, \ldots, r^T_{j_t}\} \subseteq r(T)$ that lie on the same direction of $e$.

Define the \textit{least common multiplier of a set of integer vectors with the same direction} as follows: Given $R = \{r_1, \ldots, r_l\} \subseteq \mathbb{Z}^n$ with the same direction, the least common multiplier $r$ of set $R$ is a vector $r = \lambda_1 r_1 = \ldots = \lambda_l r_l$ where $\lambda_1, \ldots, \lambda_l \in \mathbb{Z}_+$ with the least Euclidean norm. Denote $r = \text{l.c.m.}(R)$.

Given $R^S_e$ and $R^T_e$, by definition, $\text{l.c.m.}(R^S_e)$ and $\text{l.c.m.}(R^T_e)$ also lie on the same direction of $e$, so as $r_e = \text{l.c.m.}\left( \left\{ \text{l.c.m.}(R^S_e),  \text{l.c.m.}(R^T_e) \right\} \right)$.

For each extreme ray $e$ of $\cone\{r(T)\}$ and $\cone\{r(S)\}$, $r_e$ lies on the same direction of $e$. Let the set of $r_e$ for each extreme rays of $\cone\{r(T)\}$ and $\cone\{r(S)\}$ be $E = \{r_{e_1}, \ldots, r_{e_m} \} \subseteq \mathbb{Z}^n$.  Thus $\cone\{E\} = \cone\{r(T)\} = \cone\{r(S)\}$ since they have the same extreme rays.

Now define the following: 
\begin{align*}
  N(r^S_1) & := \min \left\{ \lambda \in \mathbb{Z}_+: \lambda r^S_1 = \mu_{r_{e_1}}^1 r_{e_1} + \ldots + \mu_{r_{e_m}}^1 r_{e_m}; \mu_{r_{e_1}}^1, \ldots, \mu_{r_{e_m}}^1 \in \mathbb{Z}_{\geq 0} \right\} \\
  \ldots & \\
  N(r^S_{t^S}) & := \min \left\{ \lambda \in \mathbb{Z}_+: \lambda r^S_{t^S} = \mu_{r_{e_1}}^{t^S} r_{e_1} + \ldots + \mu_{r_{e_m}}^{t^S} r_{e_m}; \mu_{r_{e_1}}^{t^S}, \ldots, \mu_{r_{e_m}}^{t^S} \in \mathbb{Z}_{\geq 0} \right\}
\end{align*}
For any real number, Let $\lfloor \cdot \rfloor$ be its round-down part and $\{ \cdot \}$ be its fractional part. Thus for any point $x \in \intcone(r(S))$, there exist $\mu_1^x, \ldots, \mu_m^x \in \mathbb{Z}_{\geq 0}$ such that
\begin{align*}
  x & = \mu_1^x r^S_1 + \ldots + \mu_{t^S}^x r^S_{t^S} \\
  & = \left( \left\lfloor \frac{\mu_1^x}{N(r_1^S)} \right\rfloor N(r_1^S) + \left\{ \frac{\mu_1^x}{N(r_1^S)} \right\} N(r_1^S) \right) r_1^S + \ldots + \left( \left\lfloor \frac{\mu_{t^S}^x}{N(r_{t^S}^S)} \right\rfloor N(r_{t^S}^S) + \left\{ \frac{\mu_{t^S}^x}{N(r_{t^S}^S)} \right\} N(r_{t^S}^S) \right) r_{t^S}^S.
\end{align*}
Let $X^S$ be set of vectors that satisfies: $x \in X^S$ if and only if
\begin{align*}
  x = \mu_1^x r^S_1 + \ldots + \mu_{t^S}^x r^S_{t^S} 
\end{align*}
where $0 \leq \mu_1^x \leq N(r_1^S) - 1, ~ \ldots, ~ 0 \leq \mu_{t^S}^x \leq N(r_{t^S}^S) - 1$. Note that $X^S$ is finite and
\begin{align*}
  \left\{ \frac{\mu_1^x}{N(r_1^S)} \right\} N(r_1^S) r_1^S + \ldots + \left\{ \frac{\mu_{t^S}^x}{N(r_{t^S}^S)} \right\} N(r_{t^S}^S) r_{t^S}^S \in X^S.
\end{align*}
Therefore, $\intcone(r(S)) = X^S + \intcone(E)$. By the same way, there exists a finite set $X^T$ such that $\intcone(r(T)) = X^T + \intcone(E)$. Thus
\begin{align*}
  S & = \bigcup_{i=1}^{k^S} P^S_i + X^S + \intcone(E) \\
  T & = \bigcup_{i=1}^{k^T} P^T_i + X^T + \intcone(E) 
\end{align*}
since $\bigcup_{i=1}^{k^S} P^S_i + X^S$ and $\bigcup_{i=1}^{k^T} P^T_i + X^T$ are union of rational polytopes, then by Proposition \ref{prop:union-mic-is-mic-int-cone}, $S \cup T$ is a MIC set.

Conversely, if $S \cup T$ is a MIC set, then $\rec S \subseteq \rec S \cup T, \rec T \subseteq \rec S \cup T$ and $\rec S \cup \rec T = \rec S \cup T$. But $\rec S$ may not equal to $\rec T$.
\chris{Guanyi to fill in the proof.}


==> proof-main-thm.tex <==
% !TEX root = ../journal-submission.tex

\section{Proof of Theorem~\ref{theorem:main}}\label{sec:full-proof-main}

\begin{proof}[Proof of Theorem~\ref{theorem:main}]
The relationships
\begin{center}
(LP) =   (LP-R)  $\subset$  (MILP)  $\subset$  (MILP-R)
\end{center}
are known but we include the proof for completeness.    By Fourier-Motzkin elimination we know that  projecting variables from a system of linear inequalities gives a new system of linear inequalities so  (LP) =   (LP-R).   There are sets in  (MILP)  that are not  convex while LP sets are convex polyhedra, so (LP) $\subset$ (MILP).  Since (LP) =   (LP-R),   (LP-R) $\subset$ (MILP).  Since a set is always a (trivial) projection of itself, (MILP)  $\subseteq$  (MILP-R).  See Williams~\cite{williams-1} for an example of a set that is in (MILP-R) but not in (MILP).  Therefore (MILP)  $\subset$  (MILP-R).

We now establish the new results

\begin{equation}\label{eq:new-results}
\textrm{(MILP-R)  =  (AC) = (AC-R) = (MIAC) =  (MIAC-R) } \subset \textrm{ (DMIAC)}.
\end{equation}
We will first show the equalities. We show in Theorem~\ref{theorem:milp-is-mic} that if a set  $S \in$ (MILP-R), then $S \in$ (AC) so  (MILP-R)  $\subseteq$  (AC).
%Now we show (AC) $\subseteq$ (AC-R) $\subseteq$ (MIAC).  
Since a set is always a (trivial) projection of itself,  (AC) $\subseteq$ (AC-R). Also it trivially follows that (AC-R) $\subseteq$ (MIAC-R) and (AC) $\subseteq$ (MIAC). Finally, since a set is a projection of itself, (MIAC) $\subseteq$ (MIAC-R). Thus, we obtain the two sequences: (MILP-R) $\subseteq$  (AC) $\subseteq$ (AC-R) $\subseteq$ (MIAC-R), and (MILP-R) $\subseteq$  (AC) $\subseteq$ MIAC $\subseteq$ (MIAC-R). To complete the proof of the equalities in~\eqref{eq:new-results}, it suffices to show that (MIAC-R) $\subseteq$ (MILP-R). Consider any $S \in$ (MIAC-R). By definition, there exists a MIAC set $C \subseteq \R^n \times \R^p\times \Z^q$ such that $S = \proj_x(C)$, where we assume $x$ refers to the space in which $S$ lies in, and we let $(y,z) \in \R^p \times \Z^q$ refer to the extra variables used in the description of $C$. In Theorem~\ref{theorem:mic-is-milp}, we show that $C \in$ (MIAC) implies $C \in$ (MILP-R), i.e., there is a MILP set $C'$ in a (possibly) higher dimension such that $C=\proj_{x,y,z}(C')$. Thus, $S = \proj_x(C) = \proj_x(\proj_{x,y,z}(C'))=\proj_x(C')$. So, $S \in$ (MILP-R).
%
%
%It follows from the lift-and-project algorithm described in Section~\ref{ss:lift-and-project} that an  (AC-R) set is an (AC) set; so (AC-R) = (AC).  Vacuously an (AC) set is also an (MIAC) set, so  (AC) $\subseteq$  (MIAC) and this combined with  (AC-R) = (AC) implies  (AC-R) $\subseteq$ (MIAC).  We now have
%
%\begin{center}
%(MILP-R)  $\subseteq$  (AC) $\subseteq$ (AC-R) $\subseteq$ (MIAC) 
%\end{center}
% We show in Theorem~\ref{theorem:mic-is-milp} that  if $S \in$ (MIAC) then $S \in$ (MILP-R) so  (MIAC) $\subseteq$  (MILP-R).  Therefore
%\begin{center}
%(MILP-R)  $\subseteq$  (AC) $\subseteq$ (AC-R) $\subseteq$ (MIAC) $\subseteq$  (MILP-R)
%\end{center}
%
%and this gives
%
%\begin{center}
%(MILP-R)  =  (AC) = (AC-R) = (MIAC).
%\end{center}
%
%Next observe that  in Section~\ref{ss:lift-and-project} we show the projection of (MIAC) set is a (MIAC) set and this proves that (MIAC) = (MIAC-R).  This gives
%\begin{center}
%(MILP-R)  =  (AC) = (AC-R) = (MIAC) =  (MIAC-R)
%\end{center}

Finally,  in Theorem~\ref{theorem:w-h-gives-projection} we show  that if  $S \in$ (MILP-R) then $S \in$ (DMIAC).  This gives (MILP-R) $\subseteq$ (DMIAC).  From  Example~\ref{ex:dmic-is-too-big} we know  (MILP-R) $\subset$ (DMIAC).  Since (MILP-R) = (MIAC-R) we now have the complete proof of~\eqref{eq:new-results}.%result
%\begin{center}
%(MILP-R)  =  (AC) = (AC-R) = (MIAC) =  (MIAC-R) $\subset$ (DMIAC).
%\end{center}
\end{proof}


